Online Convex Optimization for Sequential Decision Processes and Extensive-Form Games

Regret minimization is a powerful tool for solving large-scale extensive-form games. State-of-the-art methods rely on minimizing regret locally at each decision point. In this work we derive a new framework for regret minimization on sequential decision problems and extensive-form games with general compact convex sets at each decision point and general convex losses, as opposed to prior work which has been for simplex decision points and linear losses. We call our framework laminar regret decomposition. It generalizes the CFR algorithm to this more general setting. Furthermore, our framework enables a new proof of CFR even in the known setting, which is derived from a perspective of decomposing polytope regret, thereby leading to an arguably simpler interpretation of the algorithm. Our generalization to convex compact sets and convex losses allows us to develop new algorithms for several problems: regularized sequential decision making, regularized Nash equilibria in extensive-form games, and computing approximate extensive-form perfect equilibria. Our generalization also leads to the first regret-minimization algorithm for computing reduced-normal-form quantal response equilibria based on minimizing local regrets. Experiments show that our framework leads to algorithms that scale at a rate comparable to the fastest variants of counterfactual regret minimization for computing Nash equilibrium, and therefore our approach leads to the first algorithm for computing quantal response equilibria in extremely large games. Finally we show that our framework enables a new kind of scalable opponent exploitation approach.

==> text/cfr_lrd_perspective.tex <==
Here we try to give intuition for how one might arrive at either the LRD result
or the CFR result.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../aaai_2019/lrd_aaai_2019"
%%% End:


==> text/kuhn.tex <==
\subsection{Full description of Kuhn poker}
As an illustration, consider the game of Kuhn poker~\citep{Kuhn50:Simplified}.
Kuhn poker consists of a three-card deck: king, queen, and jack. Each player
first has to put a payment of 1 into the pot. Each player is then dealt one of the three cards, and the third is put
aside unseen. A single round of betting then occurs:
\begin{compactitem}
\item Player $1$ can check or bet $1$.
  \begin{compactitem}
  \item If Player $1$ checks Player $2$ can check or raise $1$.
    \begin{compactitem}
      \item If Player $2$ checks a showdown occurs.
      \item If Player $2$ raises Player $1$ can fold or call.
        \begin{compactitem}
          \item If Player $1$ folds Player $2$ takes the pot.
          \item If Player $1$ calls a showdown occurs.
          \end{compactitem}
        \end{compactitem}
      \item If Player $1$ raises Player $2$ can fold or call.
        \begin{compactitem}
        \item If Player $2$ folds Player $1$ takes the pot.
        \item If Player $2$ calls a showdown occurs.
        \end{compactitem}
      \end{compactitem}
\end{compactitem}
If no player has folded, a showdown occurs where the player with the higher card wins.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../aaai_2019/lrd_aaai_2019"
%%% End:


==> text/lrm_special_case.tex <==

\subsection{Best Response Differential Regret Minimization}
The previous section focused on the regret minimization algorithm corresponding
to $\gamma = 0$. Here, we investigate the other end of the spectrum, $\gamma=1$,
and we call this regret minimization scheme \emph{best response differential
  (BRD) regret minimization}; the reason for this name is that it uses the
difference in best-response value to more quickly adapt to changes in the
subtrees beneath actions.
Because BRD minimizes a tighter regret bound its guarantee on regret dominates
that of CFR. It is unclear whether this can be leveraged to prove an asymptotic
improvement in the bound for some settings.

Plugging $\gamma=1$ in \eqref{eq:losshat}, we obtain that the laminar loss at decision point $j \in \convsets$ is (we will omit the value of $\gamma$ in the parenthesis)
\[
  \losshat{j}{t}(\hat{x}) = \loss{j}{t}(\hat{x}_j) + \sum_{a\in A_j} \sum_{j' \in \childinfosets{j,a}}\!\!
  \xhat_{j,a}\big( \tinfosetvalue{j'} - \regretdiff{j'}{t} \big).
\]
%
The only difference with CFR is the presence of the negative regret differential $\regretdiff{j'}{t}$. Specifically, we discount the counterfactual loss of each action $a$ at decision point $j\in \convsets$ by keeping track of how much faster the cumulative regret is changing ``below $a$''. Intuitively, if the regret below $a$ is increasing fast, the algorithm will under-represent the loss on $a$ to encourage more exploration below $a$.

As it turns out, BRD can be expressed in a completely different way. Indeed, by definition of regret differential:
\begin{align*}
   \tinfosetvalue{j} - \regretdiff{j}{T} &= \tinfosetvalue{j} - \cumulativeregret{j}{T} + \cumulativeregret{j}{T-1} \\[-2mm]
  &= \min_{\xhat_{\subt{j}}} \sum_{t=1}^{T-1} \xhatvalue{j}{\xhat_{\subt{j}}} - \min_{\xhat_{\subt{j}}} \sum_{t=1}^{T} \xhatvalue{j}{\xhat_{\subt{j}}}\\
  &\eqdef -\partial B^T_{\subt{j}}.
\end{align*}
The term $\partial B^T_{\subt{j}}$ represents the change in the value of the best response to the cumulative loss at time $T$ versus time $T-1$, and therefore we name it \emph{best response differential}.

The value of the best-response differential can easily be computed as part of a
bottom-up traversal of the decision space: for each decision point $j$ we 
keep track of the previous best-response value, and then compute
the best response differential by choosing the point at $j$ that minimizes the
sum of the loss at $j$ and the linear term associated with best response values
below $j$. The computed value can then be passed up to the parent.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../aaai_2019/lrd_aaai_2019"
%%% End:

% LocalWords:  BRD

